Large induced subgraphs via triangulations and CMSO

We obtain an algorithmic meta-theorem for the following optimization problem. Let \phi\ be a Counting Monadic Second Order Logic (CMSO) formula and t be an integer. For a given graph G, the task is to maximize |X| subject to the following: there is a set of vertices F of G, containing X, such that the subgraph G[F] induced by F is of treewidth at most t, and structure (G[F],X) models \phi. Some special cases of this optimization problem are the following generic examples. Each of these cases contains various problems as a special subcase: 1) "Maximum induced subgraph with at most l copies of cycles of length 0 modulo m", where for fixed nonnegative integers m and l, the task is to find a maximum induced subgraph of a given graph with at most l vertex-disjoint cycles of length 0 modulo m. 2) "Minimum \Gamma-deletion", where for a fixed finite set of graphs \Gamma\ containing a planar graph, the task is to find a maximum induced subgraph of a given graph containing no graph from \Gamma\ as a minor. 3) "Independent \Pi-packing", where for a fixed finite set of connected graphs \Pi, the task is to find an induced subgraph G[F] of a given graph G with the maximum number of connected components, such that each connected component of G[F] is isomorphic to some graph from \Pi. We give an algorithm solving the optimization problem on an n-vertex graph G in time O(#pmc n^{t+4} f(t,\phi)), where #pmc is the number of all potential maximal cliques in G and f is a function depending of t and \phi\ only. We also show how a similar running time can be obtained for the weighted version of the problem. Pipelined with known bounds on the number of potential maximal cliques, we deduce that our optimization problem can be solved in time O(1.7347^n) for arbitrary graphs, and in polynomial time for graph classes with polynomial number of minimal separators.

==> beyondCmsol.tex <==
%!TEX root = MaxIndTwPropP.tex

\section{Beyond CMSO}

In this section we will give some examples showing that the previous 
described technique can be extended to problems 
that do not fit into  
the CMSO framework. 
One such example is connectivity problems where a set of terminals potentially only bounded by the size of the input is given. 
For such a problem we are not able within the standard framework of CMSO to keep track of which terminal vertex is under consideration 
as this requires $log \ n$ bits. 
Let us consider a concrete example. 

\defproblem{\midcls{}}{A graph $G$,  and a  collection   $\{T_1, T_2, \dots, T_p\}$ of terminal vertices, $T_i\subseteq V(G)$, each of size at most $\ell$.}{Find a  set $F \subseteq V(G)$ of minimum size such that  
 $G[F]$ has connected components $C_1, C_2, \dots, C_p$ and for every $1\leq i\leq p$, $T_i \subseteq C_i$.}


For example, a special case of this problem is 
\textsc{Induced Disjoint Paths}, where for a given set of $p$ pairs of terminals $x_i,y_i$, $1\leq i \leq p$, the task is to find a set of paths connecting terminals such that the vertices from different paths are not adjacent.  
Belmonte et al. \cite{BelmonteGHHKP11} have shown that \textsc{Induced Disjoint Paths} is solvable in polynomial time on chordal graphs. Before starting we will show that $G[C_i]$ is of treewidth at most $\ell$ for each $i \in [1..p]$.

\begin{lemma}\label{le:terminal_tw}
Consider a connected graph $G=(V,E)$ and a set $T \subset V$ of terminals. 
Then for every minimal vertex set $A$ where $T \subseteq A \subseteq V$ such that $G[A]$ is connected we wage that the treewidth of $G[A]$ is at most $|T|-1$.

In particular, the optimal solution $G[F]$ for problem  \midcls{} is of treewidth at most $\ell - 1$.
\end{lemma}
\begin{proof}
The proof is by induction on the cardinality of $T$. 
As the base case consider $|T|=1$ and notice that $G[T]$ is already connected and of treewidth 
zero. Assume by the induction hypothesis that the claim holds for all sets connecting terminal sets of cardinality $\ell-1$ or less and let us argue that the claim holds for terminal sets of size $\ell$. 
Let $v_1,v_2,\ldots,v_\ell$ be the vertices of $T$ and let $A' \subseteq A$ be a minimal set such that 
$\{v_1,v_2,\ldots,v_{\ell-1} \} \subseteq A'$ and $G[A']$ is connected. By the induction hypothesis 
we have that $G[A']$ is of treewidth at most $\ell-2$. 
Let $P= (v_\ell,u_1,u_2,\ldots,u_t)$ be a shortest path contained in the graph $G[A]$ from $v_\ell$ to any vertex $u_t \in N(A')$. 
%Let $A = V(P) \cup A'$ and 
Notice that $T \subseteq V(P) \cup A'$ and $G[V(P) \cup A']$ is connected, so we must have $A = V(P) \cup A'$. Thus $G[A]$ is formed by a graph $G[A']$ of treewidth at most $\ell -2$, plus the induced path $P$ such that only the vertex $u_t$ is adjacent to vertices form $A'$. A tree decomposition of width $\ell -1$ of $G[A]$ is then obtained by first adding $u_t$ to the bags of a tree decomposition of width $\ell -2$ of $G[A']$, then gluing to it a tree decomposition of the induced path $P$.
%and $A$ is a minimal set connecting $T$ as removing any vertex of $V(P) \setminus \{v_\ell\}$ 
%disconnects $v_\ell$ from $v_1$ and removing any vertex of $A'$ disconnects two vertices in 
%%$\{v_1,v_2,\ldots,v_{\ell-1} \}$ due to the minimality of $A'$. 
%If $A$ is not minimal we can simply prune it in a greedy way to obtain a minimal set. 
%Finally note that vertices of degree one can be removed from a graph of treewidth at least one 
%without decreasing the width as long as at least one edge remains, see for instance \cite{EijkhofBK07}. Remove vertices $v_\ell,u_1,u_2,\ldots u_{t-1}$ in the described 
%order until only $u_t$ remains. As $u_t$ is adjacent to a vertex of $A'$ the treewidth of $G[A' \cup \{u_t\}]$ is at least one and at most the treewidth of $G[A']$ plus one. 

The second part of the Lemma follows straightforwardly from the definition of problem \midcls.
\end{proof}


\begin{theorem}\label{theorem:disj_paths}
For a given graph $G$ with the set of potential maximal cliques $\Pi_G$ the \midcls{} problem can be solved in time $O(|\Pi_G| n^{t+O(1)})$. 
\end{theorem}
\begin{proof}

%First we need to establish some properties of an optimal solution $F$ of the \midcls{} problem that follows from Lemma \ref{le:terminal_tw} and Proposition \ref{pr:CompTr}. 
%
%\begin{observation}
%Let $F$ be a solution to the \midcls{} problem. Then 
%the treewidth of $G[F]$ is at most $\ell -1$. 
%\end{observation}
%
%This follows directly from Lemma \ref{le:terminal_tw} as each connected component is of treewidth at most $\ell -1$.

\begin{observation}\label{obs:terminalTW}
Let $F$ be a solution to the \midcls{} problem. Then 
there exists a minimal triangulation $TG$ of $G$ such that 
$|F \cap K| \leq \ell$ for each maximal clique $K$ in $TG$,
$K$ intersects at most one connected component of $G[F]$, and 
if $TD(G)$ is a clique tree of $TG$ then each connected component 
of $G[F]$ intersects maximal cliques of $TG$ that forms a subtree in $TD(G)$, and these subtrees are disjoint.
\end{observation}
The first conditions are a consequence of Lemma~\ref{le:terminal_tw} and Proposition~\ref{pr:CompTr}. The second condition comes from the fact that, for any component $C_i$ of the solution $G[F]$, the bags (cliques) of $TG$ containing vertices of $C_i$ form a connected subtree of the clique tree. Moreover, a same clique $K$ may not contain vertices of $C_i$ and $C_j$ for $i \neq j$ (because $K \cap F$ is a clique and there is no edge in $G$ from $C_i$ to $C_j$), therefore  the subtrees are disjoint.

In particular this means that connected components of the solution is distributed over disjoint subtrees 
of $TD(G)$ that are separated by edges of $TD(G)$ (corresponding to minimal separators of $G$) not intersecting the solution $F$. 
Next let us define a problem that falls within the realm of CMSO. 

\defproblem{\mcls{}}{A graph $G$,  and a terminal set $T \subseteq V$ of size at most $\ell$.}{Find a  set $X \subseteq V(G)$ of minimum size such that  $G[X]$ is connected and $T \subseteq X$.}

Property

\[\cP(G[F],X)= \{ F=X \text{ and } G[F] \text{
contains a connected component } C \text{ such that } T \subseteq C\}
\]

is CMSO-expressible since the connectivity condition is expressible in CMSO, and we need to quantify on a fix number $\ell$ of variables to ensure that $T \subseteq C$.

Problem \midcls{} is resolved by modifying the dynamic programming algorithm for \mcls{}.
In particular we will discuss how to modify the computations of the functions $\alpha,\beta,\delta,$ and $\gamma$. There are three key properties we have to ensure for a partial solution for a block $(S,C)$.

First is to ensure that every partial solution contains all terminal vertices in $C$. Using the same trick as in Theorem \ref{th:extensionswa} we only consider vertex sets $W$ that contains all terminal vertices of $S$ (resp. $\Omega$). Thus, any partial solution considered later will include all the terminal vertices.  

Next task is to ensure that terminal set $T_i$ is connected in the solution $F$. 
By Observation \ref{obs:terminalTW} it suffices to search for a solution connecting one terminal set at the time during the dynamic programming. By fixing the terminal set $T_i$ we are currently connecting the problem is reduced to \mcls{} problem. For each of the four functions $\alpha,\beta,\delta,$ and $\gamma$ used by the algorithm of \mcls{} we extend it by one extra parameter $i \in [1..p]$ indicating which terminal set we are currently connecting.  So for each integer $i$ and good triple $(S,C,\Omega)$ the algorithm of \mcls{} is used as a black box providing accepting classes for the connectivity of terminal set $T_i$. 

\ioan{From here it's sloppy}
More formally, let $\cP_i$ be the property corresponding to problem \mcls{} for the set of terminals $T_i$.
We define $\alpha(S,C,W,c,i)$ to be the minimum size solution $F \subseteq G[S \cup C]$ compatible with $(S,C,W,c)$ for property $\cP_i$ (see Definition~\ref{de:partsol}), with the supplementary condition that for any set of terminals $T_j$ intersecting $C$ with $j \neq i$, we have that $T_j$ is already in a connected component of $G[F]$. We extend in the same way the definitions of $\beta, \gamma$ and $\delta$, to ensure that sets $T_j \neq T_i$ that have been already encountered are already connected in the partial solution.

Last step is the non-connectivity between components of different terminal set including the procedure of shifting from one terminal set to the next. Observation \ref{obs:terminalTW} ensures that it is sufficient to search for solutions where at most one connected component intersect the minimal separator $S$ (resp. potential maximal clique $\Omega$). Thus, if we are connecting terminal set $T_i$ and $S$ (resp. $\Omega$) contains a terminal vertex not in $T_i$ discard all partial solutions by setting the value to $\infty$.

Let us proceed to the switch from terminal set $T_i$ to terminal set $T_j$. Terminal set $T_i$ can only be completely moved into $C \setminus S$ (resp. $C \setminus  \Omega$) if it is already connected and all maximal cliques of $TG$ (respecting solution $F$) intersecting the connected component of the solution containing $T_i$ is completely contained in $C$. In particular this means that the intersection between $C$ and maximal cliques not completely contained in $C$ do not contain vertices of the solution. 

The switch from terminal set $T_i$ to $T_j$ will be preformed when the last potential maximal clique $\Omega$ containing a vertex of the connected component for $T_i$ is reached. In the triple $(S,C,\Omega)$
we then have the property that $S$ do not intersect the solution at all. We simply adapt equation Equation \ref{eq:alpha} to preform the change given that the conditions are satisfied. 
%
%By Theorem \ref{th:extensionswa} a connected set will be produced that connects the vertices in set $T_i$ and by Observation \ref{obs:terminalSubtrees} we will reach a last potential maximal clique $\Omega$ containing a vertex of the connected component of $G[X]$ containing vertex set $T_i$. Again by Observation \ref{obs:terminalSubtrees} the transition from $\beta(S,C,\Omega,W,r,c)$ to $\alpha()S,C,W,r',c)$ given in Equation \ref{eq:alpha} need to be adapted as we are now ready to make the transition from one terminal set to the next. 


The new equation is defined as follows:\ioan{Not sure that we can do it for any class $c$; we need to switch from classes of $\cP_i$ to classes of $\cP_j$, but this also requires to "restart" the base case. I'm sure it's doable, but is it doable before Sunday ? ;-)} 
If 
$W = \emptyset$, 
$c'$ is the class accepting states for \mcls{} then 
for every $j \neq i$ and every class $c$

\begin{equation}\label{eq:alpha_swichBeyond1}
	\alpha(S,C,W,j,c) = \min \beta(S,C,\Omega,W',i,c'),
\end{equation}

where the values for $\beta(S,C,\Omega,W',i,c')$ are obtained by the partial solutions of the \mcls{} problem. 

Let us summarize. Function $\alpha(S,C,W,j,c)$ represents the minimal partial solution $F$ such that $W \subseteq F \subseteq C$, $W = S \cap F$, and very terminal set $T_i$ completely contained in $C$ is contained in the same connected component of $G[F]$. The fact that terminal vertices are always included in the set $W$, we only change from one terminal set to the next one when the first one is connected, and cases where the minimal separator (potential maximal clique) contains a vertex of a terminal set we are not currently connecting is rejected ensures that  function  $\alpha(S,C,W,j,c)$ represents what we want it to represent. The global optimal solution is retrieved from 
$\alpha(\emptyset,V,\emptyset,j,c)$ where we run over all integers for $j$ and $c$ is the accepting class.
\end{proof}




%
%
%
%. There are two key differences, the first one is switching from one terminal set to the next one during the dynamic programming and the second is to ensure that all terminal sets are connected accordingly. 
%
%In the annotated version described in Subsection \ref{ss:extension} we simply ignores vertex subsets $W$ of the minimal separator $S$ (resp. potential maximal clique $\Omega$) that do not include all the terminal vertices of $S$ (resp. $\Omega$). This adaptation of the algorithm ensures that all terminal vertices are included in any possible solution. 
%
%It remains to ensure the connectivity between terminal vertices in each set and non connectivity between vertices of different terminal sets. The connectivity is achieved through the dynamic programming for the problem \mcls{}, by simply adding a parameter to the $\alpha,\beta,\delta,$ and $\gamma$ functions indicating which terminal set we are currently connecting. There is a risk that the dynamic programming tries to use minimal separators (resp. potential maximal cliques) of that are not compatible with the solution in the sense that terminal vertices of different sets intersect the minimal separators (resp. potential maximal cliques). This is handled by simply setting the value of $\alpha(...)$ or $\beta(...)$ 
%to $\infty$ if we are currently connecting terminal set $T_r$ and the minimal separators (resp. potential maximal cliques) contains a vertex of a different terminal set. 
%
%By Theorem \ref{th:extensionswa} a connected set will be produced that connects the vertices in set $T_r$ and by Observation \ref{obs:terminalSubtrees} we will reach a last potential maximal clique $\Omega$ containing a vertex of the connected component of $G[X]$ containing vertex set $T_r$. Again by Observation \ref{obs:terminalSubtrees} the transition from $\beta(S,C,\Omega,W,r,c)$ to $\alpha()S,C,W,r',c)$ given in Equation \ref{eq:alpha} need to be adapted as we are now ready to make the transition from one terminal set to the next. 
%
%
%The new equation is defined as follows: 
%If 
%$W = \emptyset$, 
%$c$ is the class accepting states for \mcls{} then 
%
%\begin{equation}\label{eq:alpha_swichBeyond1}
%	\alpha(S,C,W,r,c) = \min \beta(S,C,\Omega,W',r',c'),
%\end{equation}
%
%else the standard equation in \mcls{} for making the transition form the $\beta$ to the $\alpha$ function is used. 
%\end{proof}
%
























%
%
%using \mcls{} as a subroutine for each terminal set defined by 
%\midcls{}. The key observation here is that a solution $X$ to the \midcls{} consist in one connected component for each of the defined terminal sets. Lemma \ref{} tells us that for a minimal triangulation $TF$ of $F$ there exists a minimal triangulation $TG$ of $G$ having $TF$ as an induced subgraph. In particular this means that vertices of different connected components of $G[F]$ are separated by a minimal separator $S$ in $TG$ such that $S \cap F = \emptyset$. Thus, we can conclude that each connected component of $G[F]$ intersects maximal cliques of $TG$ that forms a subtree of the clique tree of $TG$ and the intersection between each pairs of subtrees is empty. 
%
%
%
%\end{proof}
%
%
%
%
%Let us start by defining a similar problem that falls 
%
%
%
%Problem \midcls{} is resolved by using \mcls{} as a subroutine for each terminal set defined by 
%\midcls{}. The key observation here is that a solution $X$ to the \midcls{} consist in one connected component for each of the defined terminal sets. Lemma \ref{} tells us that for a minimal triangulation $TF$ of $F$ there exists a minimal triangulation $TG$ of $G$ having $TF$ as an induced subgraph. In particular this means that vertices of different connected components of $G[F]$ are separated by a minimal separator $S$ in $TG$ such that $S \cap F = \emptyset$. Thus, we can conclude that each connected component of $G[F]$ intersects maximal cliques of $TG$ that forms a subtree of the clique tree of $TG$ and the intersection between each pairs of subtrees is empty. 
%
%So locally we are dealing with a \mcls{} problem but one free variable is needed to keep track of the current terminal set under consideration. There are two extra details required for this algorithm. First we need an explanation of how we are moving from one terminal set to the next and secondly we have to ensure that all terminal sets completely contained in a block $(S,C)$ are connected when a partial solution is considered. 
%
%Consider now the functions $\alpha,\beta,\delta,$ and $\gamma$  defined in Section~\ref{sec:MainSection}. 
%First step is to add one more integer $r \in [0..p]$ to the tuple defining the terminal set under consideration. This means that functions $\alpha,\beta,\delta,$ and $\gamma$ considering terminal set $T_r$ only uses values of $\alpha,\beta,\delta,$ and $\gamma$ where the parameter is $r$.
%
%There is one exception to this occurs when we are shifting from one terminal set to another. 
%Remember that between each pair of connected components in $G[F]$ there exists a minimal separator $S$ 
%of $TG$ separating the two com
%
%
%
%Let us start with the main idea of the algorithm. Similar to the algorithm described in Section~\ref{sec:MainSection}
%we run over all blocks and good triples of the graph on increasing cardinality of the set $S \cup C$. Functions 
%$\alpha,\beta,\delta,$ and $\gamma$ are defined in a similar way, but the tuples are defined slightly different as we need to 
%keep track of the terminal set we are currently trying to connect. To avoid confusions terminals in $T_r$ will be called $c$-terminal
%in the meaning of connecting terminal vertices as defined by the problem. In this way the term terminal is reserved for the 
%usage in $\ell$-terminal graphs.
%Recall that in our definition of $\ell$-terminal graphs, the set of terminals is ordered. 
%The vertices of our graph are numbered from $1$ to $n$. An ordered set $W$ of vertices corresponds to
%this natural ordering over set $W$. 
%
%
%\begin{definition}\label{de:classesBeyond}
%For vertex set $W$, $c$-terminal set $T_r$, and integer $\ell$ 
%let $P_r$ be the set of partitions of 
%$T_r$ into $T^1_r,T^1_r,\ldots T^{\ell+1}_r$ and 
%$W$ into $W_1,W_2,\ldots W_{\ell}$. Then $\cal{C}$ is the set of subsets of $P_r$.
%\end{definition}
%
%
%\begin{definition}
%Given an $\ell$-terminal recursive graph $H=(F,W, E_H)$ and an integer $r$ we define function $h$ such that 
%$h(H)$ is the class $c \in \cC$ where for each partitioning 
%$T^1_r,T^1_r,\ldots T^{\ell+1}_r$ and 
%$W_1,W_2,\ldots W_{\ell}$ in $c$ there is a one to one mapping from connected components $C_1,C_2,\ldots,C_q$  of $H$ to 
%pairs $(T^i_r,W_i)$  such that $T^i_r = C_i \cap T_r$ and $W_i = C_i \cap W $ for $i \in [1..\ell]$ and $T^{\ell+1}_r = T_r \setminus F$.
%\end{definition}
%
%
%Let $G[F]$ be an induced subgraph of $G$ connecting each $c$-terminal set in an inclusion minimal way. 
%By Lemma~\ref{le:terminal_tw} each connected component of $G[F]$ is of treewidth at most $\ell$ so the treewidth of $G[F]$ is at most $\ell$.
%Then by Proposition~\ref{pr:CompTr}, there exists a (minimal) triangulation $TF$ of $G[F]$ of width at most $\ell$, and a minimal triangulation $TG$ of $G$ respecting $TF$.
%In the same way as previous sections $W = S \cap F$ (resp. $W = \Omega \cap F$) for some minimal separators $S$ (resp. potential maximal clique $\Omega$) of the minimal triangulation $TG$.
%This time there is one more restriction that follows directly from the construction of $GT$ used in Proposition~\ref{pr:CompTr}, namely that there exists an integer $r$ such that minimal separator $S$ (potential maximal clique $\Omega$) do not contain any vertex of $T_i$ or separate any pair of $c$-terminals in $T_i$ for $i \neq r$. 
%
%
%Next we need a precise definition of what a partial solution represents for this problem. 
%
%
%\begin{definition}[partial solution]\label{de:partsol_Terminal}
%Let $(S,C)$ denote a full block,
%$(S, C, \Omega)$ denote a good triple, and 
%$r$ and integer. Let $W \subseteq S$ (resp. $W \subseteq \Omega)$ be a vertex subset of size at most $\ell$ and $c$ be a class in $\cC$. 
%We say that $G[F]$ is a \emph{partial solution compatible with} $(S,C, W,r, c)$ (resp. with  $(S, C, \Omega, W,r, c)$) if:
%\begin{enumerate}
%\item $F \subseteq S \cup C$, $W = F \cap S$, and $T_r \cap S \subseteq W$ (resp. $W = F \cap \Omega = W$, and $T_r \cap \Omega \subseteq W$);
%%\item $T_i \cap S = \emptyset$ (resp. $T_i \cap \Omega = \emptyset$)for each $i \neq r$;
%\item $T_i \subseteq C'$ for some connected component $C'$ of $G - S$ (resp. $G- \Omega$) for each $i \neq r$;
%\item for every $i \neq r$ such that $T_i \subseteq C$ there exists a connected component $C_i$ of $G[F]$ such that $T_i \subseteq C_i$ and $C_i \cap T_j = \emptyset$ for $j \neq i$;
%\item the $\ell$-terminal recursive graph $H=(F, W, E(G[F]))$ satisfies $c = h(H)$;
%\item there is a  triangulation $TF$ of $G[F]$ of width at most $\ell$ and a minimal triangulation $TG$ of $G$ respecting $TF$, such that $S$ is a minimal separator (resp. $\Omega$ is a maximal clique) of $TG$.
%\end{enumerate}
%\end{definition}
%%The third condition implies that $W$ induces a clique in the triangulation $TF$ of $G[F]$. 
%%For the second point, note that $H$ is a $(t+1)$-terminal recursive graph by Proposition~\ref{pr:tw_expr}.
%
%Let $\alpha(S,C,W,r,c)$ denote the size of a smallest partial solution compatible with $(S,C, W,r, c)$ and $\beta(S, C, \Omega, W,r, c)$ denote the size of the smallest partial solution compatible with $(S, C, \Omega, W,r, c)$.
%%We also define 
%%\begin{itemize}
%%\item $(S,C)$ denotes a full block and $(S, C, \Omega)$ denotes a good triple.
%%\item $\alpha(S,C,W,c)$ denotes the size of a largest induced $(t+1)$-terminal subgraph $H=(F,W,E(G[F]))$ such that $F$ is contained in the block $(S,C)$, $F$ intersects $S$ exactly in $W$ and the class $h(H)$ of this partial solution is $c$.
%%\item $\beta(S, C, \Omega, W, c)$ is the size of a largest induced $(t+1)$-terminal subgraph $H=(F,W,E(G[F]))$ such that $F$ is contained in the block $(S,C)$, $F$ intersects $\Omega$ exactly in $W$ and the class $h(H)$ of this partial solution is $c$. 
%%\end{itemize}
%% Observe that in the $\beta$ function,  $W$ represents the intersection between the partial solution and the potential maximal clique $\Omega$, while in the definition of the $\alpha$ function, $W$ is the intersection of the partial solution with the minimal separator $S$. 
%If partial compatible solutions do not exist, we simply set the corresponding value of $\alpha$ or $\beta$ to $\infty$.
%
%\subsection{The algorithm}
%
%
%The algorithms proceeds by dynamic programming on full blocks and good triples. By~\cite{FKTV08}, the number of good triples is $O(n|\Pi_G|)$.
%The blocks are first sorted by size. For each block $(S,C)$ by increasing size, we first compute the values $\beta(S,C,\Omega,\dots)$ from values $\alpha(S_i,C_i,\dots)$ corresponding to smaller blocks, then we compute the values $\alpha(S,C,\dots)$ from values $\beta(S,C,\Omega,\dots)$, in the same way as described in Algorithm~\ref{al:mainalgBeyond}. 
%
%		\begin{algorithm}[H]
%		\caption{\midcls{} }\label{al:mainalgBeyond}
%		\SetKwInput{Input}{Input}
%		\SetKwInput{Output}{Output}
%		\SetKw{all}{all}
%		%\DontPrintSemicolon
%		\Indm
%		%\bf{Algorithm {\sc Maximum Induced} ${\mathcal G}(t,\cP)$\\}
%		\Input{graph $G$, $\Pi_G$,  collection   $\{T_1, T_2, \dots, T_p\}$ of $c$-terminal vertices, classes $\cC$ and functions $h$}
%		\Output{minimal solution to the \midcls{} problem}
%		\Indp
%		\smallskip
%		Order all full blocks by inclusion\;
%		\ForAll{full blocks $(S,C)$ in this order}
%		{
%			\ForAll{good triples $(S,C,\Omega)$, \all $W \subseteq \Omega$ of size $\leq \ell$, \all $r \leq p+1$, and \all $c \in \cC$}
%			{
%				\eIf{$\Omega = S \cup C$}
%				{
%					Compute $\beta(S,C,\Omega,W,r,c)$ using Equation~\ref{eq:base_caseBeyond}\;
%				}
%				%\Else
%				{
%					Compute $\beta(S,C,\Omega,W,r,c)$ using Equations~\ref{eq:deltaBeyond}, \ref{eq:gamma1Beyond}, \ref{eq:gammaiBeyond},  and~\ref{eq:betaBeyond} \;
%				}
%			}
%			\ForAll{$W \subseteq S$ of size $\leq \ell$, \all $r \leq p+1$, and \all $c \in \cC$}
%			{
%				Compute $\alpha(S,C,W,r,c)$ using Equations~\ref{eq:alpha_swichBeyond1} and \ref{eq:alpha_swichBeyond2}\;
%			}
%
%		}
%		Compute the optimal solution using Equation~\ref{eq:finalBeyond}\;
%		\end{algorithm}
%
%
%\paragraph{The base case.} The base case consists in minimal full blocks $(S, C, \Omega)$, in which case $\Omega = S \cup C$ by~\cite{BoTo01}. In this case, for any partial solution $G[F]$ compatible with $(S,C,\Omega,W,r,c)$ we must have $F=W$, hence $G[W]$ corresponds to partial solution and using Definition~\ref{de:partsol_Terminal} we can simply check if $G[W]$ is a valid partial solution. 
%
%\begin{equation}\label{eq:base_caseBeyond}
%\beta(S, C, \Omega, W,r, c) =  \left\{ \begin{array}{l l}
%		|W| & \text{~if~}|W|\text{~is a partial solution by Definition~}\ref{de:partsol_Terminal},\\
%		\infty &\text{~otherwise} 
%		\end{array}
%		\right.
%\end{equation}
%
%The computation of each value $\beta(S, C, \Omega, W,r, c)$ corresponding to a base case takes $O(n)$ time, because we have to store the value in a table indexed by $(S, C, \Omega,r,c)$ and 
%check some properties of all $c$-terminal vertices. 
%The number of good triples is $O(n|\Pi_G|)$ so altogether these computations take $O(n^{t+3}|\Pi_G|)$ time. 
%%(Actually, one can prove by a more careful analysis that the number of good triples corresponding to base cases is at most $n$.)
%
%%The correctness comes from the fact that, in this base case, the only possible partial solution compatible with $(S, C, \Omega, c)$ is $G[W]$.
%
%\paragraph{Computing $\alpha$ from $\beta$.}
%Our goal is to compute $\alpha(S,C,W,r,c)$ from values $\beta(S,C,\Omega,W',r',c')$ such that $(S,\Omega,C)$ is a good triple and $W = W' \cap S$. 
%
%Consider any partial solution $G[F]$ compatible with $(S,C,W,r,c)$. Let $TF$ be a  triangulation of $G[F]$ like in Definition~\ref{de:partsol_Terminal} and let $TG$ be a  minimal triangulation of $G$ respecting $TF$. Let $\Omega$ be the  maximal clique of $TG$ such that $S \subseteq \Omega \subseteq S \cup C$ (this clique is unique by~\cite{BoTo01}) and take $W' = \Omega \cap F$.  Note that $G[F]$ is also a partial compatible solution for $(S,C,\Omega, W',r', c')$ where $c'$ is the homomorphism class of the $\ell$-terminal graph $H' = (F, W', E(G[F]))$. Also observe that  the $\ell$-terminal graph $H=(F,W,G[F])$ is obtained from $H'$ by the unary composition function $f(W',W)$ that consists in removing $W' \sm W$ from the set of terminals, and possibly renumbering the remaining terminals.
%Therefore  $\odot_{f(W',W)}(c')=c$. For a specific partitioning it will simply mean that if $(T^i_r,W_i)$ are subsets in a partitioning in $c'$ then this will be 
%$(T^i_r,W_i \setminus (W' \setminus W))$.
%Moving from $\beta$ to $\alpha$ is the only equation that allows us to change the value of $r$, but this can only happen if all $c$-terminals of $T_r$ is already connected and there is only a single 
%connected set that remains. 
%
%\begin{lemma}\label{le:a_from_b_swich}
%If 
%$W = \emptyset$, 
%$c$ is the class consisting of the partitioning where $T^{\ell+1}_r = T_r$,
%$W' \neq \emptyset$, and 
%$c'$ is the class consisting of the partitioning where there exits an integer $i$ such that $T^i_r = T_r$ and $W_i = W'$, then use
%
%\begin{equation}\label{eq:alpha_swichBeyond1}
%	\alpha(S,C,W,r,c) = \min \beta(S,C,\Omega,W',r',c'),
%\end{equation}
%else use 
%\begin{equation}\label{eq:alpha_swichBeyond2}
%	\alpha(S,C,W,r,c) = \min \beta(S,C,\Omega,W',r,c'),
%\end{equation}
%where the maximum is taken over all good triples $(S,C,\Omega)$, all subsets $W' \subseteq \Omega$ of size at most $\ell$ such that $W' \cap S = W$ and all classes $c' \in \cC$ such that 
%$\odot_{f(W',W)}(c')=c$ and $r'$ is any integer in $[1..p+1]$. 
%\end{lemma}
%\begin{proof}
%Equation~\ref{eq:alpha_swichBeyond1} corresponds to the case where $c$-terminal set $r'$ has already been connected in a minimal way and we are looking at the separator $S$ having an 
%empty intersection with the target solution $F$. In this case we simply start the construction of the new $c$-terminal set $r$ which do not intersect $S \cup C$ at all. 
%Equation~\ref{eq:alpha_swichBeyond2} simply emulates the corresponding equation given in Section~\ref{sec:MainSection}.
%\end{proof}
%
%Integer $r$ is simply indicating the current $c$-terminal set we want to connect in a minimal way. 
%Shifting from one $c$-terminal set to another is only done after the previous set is connected and we have a separator $S$ not intersecting the solution. 
%Such a separator will clearly exists as $TF$ consist of several connected components and $TG$ respects $TF$. All remaining equations will only deal 
%with a single $c$-terminal set $T_r$ and thus $r$ will be the same on both sides of the equations. 
%
%
%% 
%% For computing all values $\alpha(S,C,W,r,c)$ from values $\beta(S,C,\Omega,W',r',c')$, we proceed in a slightly different and more efficient way than the one described in the Algorithm~\ref{al:mainalg}. When $\beta(S,C,\Omega,W',r',c')$ is computed (lines 5 or 7 of the algorithm), if $\odot_{f(W',W)}(c')=c$ we simply update the value of $\alpha(S,C,W,r,c)$ by taking the maximum between the previous value and $\beta(S,C,\Omega,W',r',c')$. This only costs an extra $O(n)$ for each quintuple $(S,C,\Omega,W',r',c')$. The number of such quintuples is $\cO(n^{t+2}|\Pi_G|)$, thus the total cost of these computations is  $\cO(n^{t+3}|\Pi_G|)$.
%
%
%
%\paragraph{Computing $\beta$ from $\alpha$.}
%We now compute $\beta(S,C,\Omega,W,r,c)$ from values $\alpha(S_i, C_i, W_i,r, c_i)$ where $C_i$, $1 \leq i \leq q$ are the connected components of $G[C \setminus \Omega]$, 
%$S_i = N_G(C_i)$, $W_i = C_i \cap S_i$ and $c_i$ are classes (still to be guessed). 
%
%Intuitively, let $H = (F, W, E_H)$ be an optimal partial solution for  $\beta(S,C,\Omega,W,r,c)$ and let $H_i = (F_i, W_i, E_i)$ be its trace on the smaller block $(S_i, C_i)$. Hence $F_i = F \cap (S_i \cup C_i)$, $W_i = W \cap S_i$ and $E_i = E(G[F_i])$. Observe that $H$ is obtained from the smaller $H_i$s as follows:
%\begin{itemize}
%\item on each $H_i$, we introduce the terminals of $W \sm W_i$, obtaining a graph $H_i^+ = (F_i \cup W, W, E^+_i)$ with $W$ as set of terminals and with $E^+_i = E(G[F_i \cup W])$ as edge set.
%\item we perform a sequence of joins, gluing one by one $H^+_1, H^+_2,\dots, H^+_p$ on the same set of terminals $W$.
%\end{itemize}
%
%Formally, let us first define $\delta_i(S, C, \Omega, W,r,c_i^+)$ to be the size of the largest partial solution $G[F^+_i]$ compatible with $(S,C,\Omega,W,r,c^+_i)$ such that $F^+_i \subseteq \Omega \cup C_i$. (This partial solution was denoted above by $H^+_i$, and  $F^+_i$ corresponds to $F_i \cup W$.) Consider the composition operation $in(W_i,W)$ which takes two $\ell$-terminal graphs, with terminal sets $W_i$ and $W$ respectively, 
%and composes them into a new $\ell$-terminal graph having $W$ as set of terminals. In the gluing operation, terminal number $j$ of $W_i$ is glued on terminal number $k$ of $W$ if and only if they correspond to the same vertex of $G$. Hence, this composition function $in(W_i,W)$ only depends on $W_i$ and $W$. Let $c_W$ be the homomorphism class of the base $\ell$-terminal graph corresponding to $G[W]$, thus having $W$ as set of terminals. %\yv{We are using terminals in two different meanings here. }
%
%\begin{lemma}
%\begin{equation}\label{eq:deltaBeyond}
%	\delta_i(S, C, \Omega, W,r, c_i^+) = \min_{c_i\text{~s.t.~} \odot_{in(W_i,W)}(c_i,c_W) = c^+_i} \alpha(S_i,C_i,W_i,r, c_i) + |W \setminus W_i|.
%\end{equation}
%\end{lemma}
%\begin{proof}
%% Let $G[F^+_i]$ be a maximal partial solution compatible with $(S,C,\Omega,W,c^+_i)$ such that $F^+_i \subseteq \Omega \cup C_i$. 
%% Denote $F_i = F^+_i \cap (S_i \cup C_i)$. Observe that $G[F_i]$ is a partial solution compatible with $(S_i,C_i,W_i, c_i)$ for some class $c_i$, and this class must 
%% satisfy $\odot_{in(W_i,W)}(c_i,c_W) = c^+_i$. 
%% Hence $\delta_i(S,\Omega,C,W,c_i^+)$ is at most equal to the right-hand side of the equation.
%% 
%% Conversely, take a maximum partial solution $G[F_i]$ contained in $S_i \cup C_i$, compatible with $(S_i,C_i,W_i, c_i)$, where $ \odot_{in(W_i,W)}(c_i,c_W) = c^+_i$. Then $(F_i \cup W, W, E(G[F_i \cup W]))$ is a partial solution compatible with  $(S,C,\Omega,W,c^+_i)$, and the equality follows.
%\end{proof}
%
% We introduce another notation $\gamma_i(S,C,\Omega,W,r,c)$, corresponding to the largest partial solution compatible with $(S,C,\Omega,W,r,c)$, contained into $\Omega \cup C_1 \cup \dots \cup C_i$. It corresponds to the gluing of some partial solutions $H_1^+, \dots H_i^+$. 
% 
% \begin{lemma}
% Function $\gamma_i$ is computed as follows.
%%\begin{itemize}
%%\item 
%\begin{equation}\label{eq:gamma1Beyond} 
%	\gamma_1(S,C,\Omega,W,r,c) = \delta_1(S,\Omega,C,W,r,c)
%	\end{equation}
%%\item 
%For any $i$, $2 \leq i \leq q$, 
%\begin{equation}\label{eq:gammaiBeyond}
%\gamma_i(S,C,\Omega,W,r,c) = \min_{c',c''} \gamma_{i-1}(S,C,\Omega,W,r,c') + \delta_i(S,\Omega,C,W,r,c'') - |W|,
%\end{equation}
% over all characteristics $c',c''\in \cC$ such that $\odot_{g(W)}(c',c'') = c$, where $g(W)$ is the composition function corresponding to a join operation on $W$. I.e., the matrix $m(g(W))$ of $g(W)$ has $|W|$ rows, and $m_{j,1}(g(W))=m_{j,2}(g(W))=j$ for each row $j$.
%%\end{itemize}
%\end{lemma}
%\begin{proof}
%The proof is trivial for $\gamma_1$.
%
%Now for any $F \subseteq \Omega \cup C_1 \cup \dots \cup C_i$, note that $G[F]$ is a partial solution compatible with $(S,C,\Omega,W,r,c)$ if and only if $F \setminus C_i$ (resp. $F \setminus (C_1 \cup \dots \cup C_{i-1})$) are partial solutions compatible with  $(S,\Omega,C,W,r,c'')$ (resp. $(S,C,\Omega,W,r,c')$) and $\odot_{g(W)}(c',c'') = c$. 
%\end{proof}
%
%The following result is a direct consequence of the definition of $\beta$ and $\gamma$ functions.
%\begin{lemma}
%\begin{equation}\label{eq:betaBeyond}
%\beta(S,C,\Omega,W,r,c) = \gamma_q(S,C,\Omega,W,r,c).
%\end{equation}
%\end{lemma}
%
% 
%We claim that computing, for a fixed tuple $(S,C,\Omega,r,W)$, the values $\beta(S,C,\Omega,W,r,c)$ from values $\alpha$,  takes $O(m)$ time. Again by~\cite{FKTV08}, the smaller blocks $(S_i,C_i)$ can be listed in $O(m)$ time. For each $i$, the computation of  function $\delta_i(S,\Omega,C,W,r,c_i^+)$ takes $O(|S_i|+|C_i|)$ time, because we need to access the values $\alpha(S_i,W_i,C_i,r,c_i)$. The sum of these values is at most $n+m$~\cite{FKTV08}.
%
%
%Computing $\gamma_i(S,C,\Omega,W,r,c)$ from values $\gamma_{i-1}$ and $\delta_i$ can be done in $O(n)$ time for each $i$.
%Therefore the running time of the algorithm is $n^2$ times the number of quintuples $(S, C, \Omega, W, c)$, that is $O(|\Pi_G|n^{t+4})$.
%
%
%\paragraph{The global solution.} It can be obtained by considering the (special) full block $(\emptyset, V)$. 
%\begin{lemma}
%The solution size is 
%\begin{equation}\label{eq:finalBeyond}
%\min_c \alpha(\emptyset, V, \emptyset,\ell+1, c),
%\end{equation}
% over all accepting classes $c$, i.e., classes such that $(h(G)=c)$ implies that all $c$-terminal sets are connected in a minimal way. 
%\end{lemma}
%\begin{proof}
%By definition of regular properties and of $\alpha(\emptyset, V, \emptyset,\ell+1, c)$, our problem has a solution of size at most  $\min_c \alpha(\emptyset, V, \emptyset,\ell+1, c)$ over accepting classes $c$.
%
%Let $G[F]$ be a maximum size solution for our problem. By Proposition~\ref{pr:CompTr}, this solution is compatible with $\alpha(\emptyset, V, \emptyset,\ell+1, c)$ for the class $c$ of the $\ell$-terminal graph graph $(F, \emptyset, E(G[F]))$, which achieves the proof of the lemma.
%\end{proof}
%%
%%This latter computation takes constant time. 
%
%%The total running time of the algorithm is $O(|\Pi_G|n^{t+4})$. Note that, instead of keeping the size of the largest solution $G[F]$, we could explicitly store the vertex subset $F$.
%
%%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%% 
%% 
%% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % YV: Old version 19.06 
% %%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{proof}(Sketch of proof)
% Many of the arguments are the same as the one given in Section \ref{sec:MainSection} so we will only highlight the main differences and key points. 
% 
% By Lemma \ref{le:terminal_tw} each connected component of $G[F]$  
% for a solution $F$ of the \midcls{} problem is of treewidth at most $\ell-1$ 
% and thus there exists a minimal triangulation $TF$ of $G[F]$ with a maximum clique of size $\ell$.
% As described in Proposition \ref{pr:CompTr} there exists a minimal triangulation $TG$ of $G$ respecting $TF$, meaning that a maximal connected component of $TG$ intersects at most one connected component in $G[F]$ and the intersection is of size at most $\ell$. 
% 
% We will now describe how to solve the \midcls{} by extending the dynamic programming by some polynomial size information provided by the
% minimal separators and potential maximal cliques of $TG$. In the same fashion as Section \ref{sec:MainSection} 
% we define function $\alpha,\beta, \delta$, and $\gamma$ using slightly different tuples. 
% 
% %As before let $\Pi_G,\Delta_G$ be the set of all potential maximal cliques and minimal separators of $G$. 
% 
% 
% In the same way as before $W$ will represent the intersection between the minimal separator $S$ or potential maximal clique $\Omega$  and the potential solution. At most one connected component $C_r$ of $G[F]$ can intersect $S$ or $\Omega$ so let $r$ denote the index of this terminal set being a subset of $C_r$. Given the previous structure we know that for any minimal triangulation of $G$ respecting the solution we have that $C_i \cap S = \emptyset$ and $C_i \cap \Omega = \emptyset$ for each $i \neq r$. 
% 
% Let $\cal{C}$ be a finite set of which the cardinality only depends on $|T_r|$ and $|W|$, but as both these sets are bounded by $\ell$ 
% the cardinality of $\cal{C}$ is bounded by a function of $\ell$.
% %Each class $c \in \cal{C}$ represents some partiall connectivety between terminals in $T_r$. 
% Let $T_a,T_b$ be a partitioning of $T_r$ into two sets,
% $T'_1,T'_2,\ldots T'_y$ be a partitioning of $T_a$ into $y$ sets, and 
% $W_1,W_2,\ldots W_y$ be a partitioning of $W$ into $y$ sets where $y = \ell$. 
% Note that some of the sets in a partition might be empty. 
% For each subset of these partitionings  we define a class $c \in \cal{C}$.
% If $T_a = T'_1 = T_r$ and $W_1 = W$ an element in the class $c$ it will be defined as an accepting class. 
% 
% 
% % YV: Maybe we should add an explanation for the partitionings
% 
% Let $\alpha(S,C,W,r,c)$ be the size of the minimum number such that for 
% each partitioning $T'_1,T'_2,\ldots T'_y$ and 
% $W_1,W_2,\ldots W_y$ 
% (where $T_r \cap (S \cup C)$ )
% contained in class $c$ there exists a vertex set $F'$ such that 
% $|F'| = \alpha(S,C,W,r,c)$,
% $F' \subseteq W \cup C$, 
% $T_i \cap (C \cup S) \subseteq F'$ for each $i \in [1..p]$,
% if $T_i \cap C \neq \emptyset$ and $i \neq r$ then $T_i \subseteq C'$ for some connected component $C'$ of $G[F']$, 
% $G[F']$ contains no path from $u$ to $v$ where $u \in T_i$ and $v \in T_j$ 
% for $i \neq j$.
% 
% %  and class $c$ 
% %is the set of partitionings such that  
% %$T_a = F' \cap T_r$,
% %the partitioning $W_1,W_2,\ldots W_y$ of $W$ into connected components of $G[F']$, and finally the partitioning $T'_1,T'_2,\ldots T'_y\}$ of $T_a$ into 
% %connected components of $G[F']$.
% 
% Function $\beta(S,C,\Omega,W,r,c)$ is defined in the same way as $\alpha$ 
% with the exception that $W$ is a subset of $\Omega$ and not $S$.
%  
% Base case will be the $\beta(S,C,\Omega,W,r,c)$ functions where $S \cup C = \Omega$. Running over all subsets $W$ of $\Omega$ and classes in $\cal{C}$ we can simply find the optimal value for $\beta(S,C,\Omega,W,r,c)$ as each of the properties are eacy to check given $F'$. 
% 
% The following formula will be used to obtain $\alpha$ values from $\beta$ 
% values of the same $(S,C)$ block:
% 
% $$\alpha(S,C,W,r,c) = \min{\beta(S,C,\Omega,W',r',c')}$$ 
% 
% where the following conditions are satisfied. 
% First $W = W' \cap S$ and let $F_a = F_r \cap (S \cup C)$.
% If class $c'$ contains partitioning 
% $T'_1,T'_2,\ldots T'_y\}$, and 
% $W_1,W_2,\ldots W_y$ 
% then $c$ contains the partitioning 
% $T''_1,T''_2,\ldots T''_y\}$, and 
% $W'_1,W'_2,\ldots W'_y$ where 
% $T'_i = T''_i$ for each $i \in [1..y]$ and 
% $W_i = W'_i \cap S$ for each  $i \in [1..y]$ and further more 
% Vertex set $W_i$ is only empty if $W'_i$ is empty or $i = 1$ and $W = \emptyset$ and $T'_1 = T_r$. 
% %If this is not the case then $\beta(S,C,\Omega,W',r',c')$ is not considered in the minimization. 
% 
% Let us embark on the transission from $\alpha$ to $\beta$ functions. 
% Here two intermediate functions called 
% $\delta_i(S,C,\Omega,W,r,c_i^+)$ and 
% $\gamma_{i}(S,C,\Omega,W,r,c)$ are required. 
% To define these let $C_1,C_2,\dots,C_z$ be the connected components 
% of  $G[C \setminus \Omega]$. 
% Function $\delta_i(S,C,\Omega,W,r,c_i^+)$ provides the minimum partial solution obtained from component $C_i$ and $W \subset \Omega$ consistent with $c$ and 
% $\gamma_{i}(S,C,\Omega,W,r,c)$ provides the minimum partial solution from 
% components $C_1$ to $C_i$ and $W \subset \Omega$ that are consistent with $c$. 
% 
% First step is from $\alpha$ to $\delta$ functions is defined as follows: 
% 
% $$\delta_i(S,C,\Omega,W,r,c_i^+) = \min{\alpha(S_i,C_i,W',r,c)}$$
% 
% where 
% $S_i = N_G(C_i)$,
% vertex set $W' \subseteq W$,
% let $T'_1,T'_2,\ldots T'_y\}$ and 
% $W_1,W_2,\ldots W_y$ be a 
% 
% 
% 
%  
%  
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% 
% $c$ is the class obtaiend from $c'$ when mapping each connected component 
% 
% 
% In the same way as before we let $\alpha(S,C,W,r,c) = \max \beta(S,C,\Omega,W',r,c')$ 
% YV: Explain the link between these two. 
% as this is the equivalent to the forget operation in nice tree decompositions. 
% 
% The opposite direction form $\alpha$ to $\beta$ requires two new functions $\delta$ and $\gamma$.
% Let $C_1,C_2,\ldots,C_z$ be the connected components of $C \setminus \Omega$.
% Let $\delta_i(S, C, \Omega, W,r,c_i^+)$ represent the minimal partial solution of $F \cap (\Omega \cup C_i)$ such that every terminal set $T_j$ completely contained in $C \setminus \Omega$ is connected, 
% there are no path between vertices of terminal sets $T_{j'}$ and $T_j$ for $j' \neq j$ 
% in $F \cap (\Omega \cup C_i)$, $W$ is the intersection between $F$ and $\Omega$.
% 
% The function is as before : 
% $\delta_i(S,\Omega,C,W,r,c_i^+) = \alpha(S_i,C_i,W',r',c') + something $.
% 
% Next we need $\gamma_i(S,C,\Omega,W,r,c)$ represent the minimal partial solution of $F \cap (\Omega \cup \bigcup_{j = 1}^{i} C_j)$ such that every terminal set $T_{j'}$ completely contained in $\bigcup_{j = 1}^{i} C_j$ is connected, and 
% there are no path between vertices of terminal sets $T_{j'}$ and $T_j$ for $j' \neq j$ 
% in $F \cap (W \cup \bigcup_{j = 1}^{i} C_j)$, $W$ is the intersection between $F$ and $\Omega$.
% 
% Like before function $\gamma_i$ is computed as follows.
% \begin{itemize}
% \item $\gamma_1(S,C,\Omega,W,r,c) = \delta_1(S,\Omega,C,W,r,c)$.
% \item For any $i$, $2 \leq i \leq p$, $$\gamma_i(S,C,\Omega,W,r,c) = \max_{c',c''} \gamma_{i-1}(S,C,\Omega,W,r,c') + \delta_i(S,\Omega,C,W,r,c'') - |W|,$$ over all characteristics $c',c''\in \cC$ such that $\odot_{g(W)}(c',c'') = c$, where $g(W)$ is the composition function corresponding to a join operation on $W$. I.e., the matrix $m(g(W))$ of $g(W)$ has $|W|$ rows, and $m_{j,1}(g(W))=m_{j,2}(g(W))=j$ for each row $j$.
% \end{itemize}
% 
% 
% 
% \end{proof}

%
%==========TO INTRO AND PRELIMINARY ======

%TO ADD:  Proposition on  Enumeration minimal separators
%The following result will be used to list all minimal separators of
%a graph.

%

%We can also demand, for example, that every connected component in \idclp{} can be an 
%induced path  of odd length, a tree, an outerplanar graph, etc. 
%A special variant of this problem, known as \textsc{Odd Path}, is to decide if two given vertices can be connected by a path of odd length, is known to be NP-complete \cite{Bienstock91}.
% Polynomial time algorithms for   \textsc{Odd Path} were known for several graph classes, including chordal  \cite{ArikatiP93} and  circular-arc graphs \cite{ArikatiRM91}. 

%

%
%TO CHECK: $k$-in a path, $k$-in a tree, $k$ in a cycle, $k$ in a graph of treewidth $\leq t$.

%

%

%

%Algorithms on special graph classes: limits of tractability. First limit studies which range of NP complete problems are solvable on specific classes of graphs. The other, what is the ultimate generalization of the graph class allowing to do solve this problem.
%We contribute in both directions. 

%
%Chordal graphs:
%Yannakakis and Gavril \cite{YannakakisG87}: 
% the problems of finding maximum and connected maximum $k$-colorable subgraphs in chordal graphs. The problems are polynomially solvable when $k$ is fixed and NP-hard when $k$ is not fixed. As a special case,  in polynomial time the maximum induced tree and forest of a chordal graph.  Note: in chordal graph $k$-colorable subgraph is of treewidth $k$.

%
%Circular-arc graphs: Independent set 
%\cite{Gavril74}.

%Perfect graphs: Independent set ellipsoid method. 

% 

%%
%%
%%Weakly chordal:  the number of edges in the complement  Bouchitt{\'e}  and  Todinca \cite{BoTo01}
%%
%%circular-arc:  $2n^2 -3n$ Kloks, Kratsch, and Wong \cite{KloksKW98}
%%
%%
%%
%%$d$-trapezoid  Kratsch \cite{Kr96} $(2n-3)^{d-1}$, see also \cite{brandstadt1999graph}.

%

%

%It means that the following problems are solvable in poynomial time on these classes of graphs:

%- finding a maximum induced (connected) subgraph with vertex degree at most $\ell$

%- Maximum induced subgraph with chromatic index $\ell$.

%
%Robust algorithms, recognition of $d$-trapezoid graph is NP-hard.

%
%=================

%

%Let $H_{k,k}$ be a $(k\times k)$-grid, i.e. the Cartesian product of two paths  $P_k$.

%\begin{proposition}[\cite{RobertsonS3}]\label{prop:RS_grid}
%For every integer $k>0$ there exists $g(k)>0$ such that every graph of treewidth more than $g(k)$ contains a subdivision of $H_{k,k}$
%\end{proposition}

%Bounds on $g(k)$ \cite{RobSeymT94} and mention new paper of Seymour. 

%
%\begin{proposition}[\cite{Thomassen88}]\label{prop:Thomas_grid}
%For every integers $k,m>0$ there exists an integer $h(k,m)>0$ such that every subdivision of 
%$H_{h(k,m),h(k,m)}$  contains a subdivision of $H_{k,k}$ such that each edge of  $H_{k,k}$ is a path 
%of length $0\imod{m}$.
%\end{proposition}

%
%\medskip

%Let $\mathcal{ F}$ be a graph family. We say that
%$\mathcal{ F}$ has the Erd\H{o}s-P\'{o}sa property 
%if for any graph $G$,
%the minimum vertex covering of all 
%subgraphs of $G$ isomorphic to a member of $\mathcal{ F}$
%is bounded by a function $f$ of the maximum
%packing of subgraphs   isomorphic to a member of $\mathcal{ F}$.

%

%\begin{proposition}[\cite{Thomassen88}]
%Let $\cF$ be a family of connected graphs and $G_0$ a connected planar graph of maximum degree at most $3$ and $m$ any natural number. If $\cF$ contains all those subdivisions of $G_0$ in which each edge of $G_0$ corresponds to a path of length $0\imod{m}$, then $\cF$ has the Erd\H{o}s-P\'{o}sa property. 
%\end{proposition}

%Robertson-Seymour.
%Chekury-Chuzhoy \cite{ChekuryCh13}. 
%\cite{ChekuriCh_grid13}

%


%
%
%$\mathcal{ H}$-subgraphs in $G$ (by $\mathcal{ H}$-subgraph of $G$ we mean
%any subgraph of $G$ that belongs to $\mathcal{ H}$).
%
%
%A graph family $\cF$ has the Erd\H{o}s-P\'{o}sa property if there exists a function $f(k)$ such that any graph $G$ contains either $k$ disjoint subgraphs each isomorphic to a member of $\cF$   
%Thomassen \cite{Thomassen88}



